GAMMA Challenge:Glaucoma grAding from Multi-Modality imAges

Color fundus photography and Optical Coherence Tomography (OCT) are the two most cost-effective tools for glaucoma screening. Both two modalities of images have prominent biomarkers to indicate glaucoma suspected. Clinically, it is often recommended to take both of the screenings for a more accurate and reliable diagnosis. However, although numerous algorithms are proposed based on fundus images or OCT volumes in computer-aided diagnosis, there are still few methods leveraging both of the modalities for the glaucoma assessment. Inspired by the success of Retinal Fundus Glaucoma Challenge (REFUGE) we held previously, we set up the Glaucoma grAding from Multi-Modality imAges (GAMMA) Challenge to encourage the development of fundus \& OCT-based glaucoma grading. The primary task of the challenge is to grade glaucoma from both the 2D fundus images and 3D OCT scanning volumes. As part of GAMMA, we have publicly released a glaucoma annotated dataset with both 2D fundus color photography and 3D OCT volumes, which is the first multi-modality dataset for glaucoma grading. In addition, an evaluation framework is also established to evaluate the performance of the submitted methods. During the challenge, 1272 results were submitted, and finally, top-10 teams were selected to the final stage. We analysis their results and summarize their methods in the paper. Since all these teams submitted their source code in the challenge, a detailed ablation study is also conducted to verify the effectiveness of the particular modules proposed. We find many of the proposed techniques are practical for the clinical diagnosis of glaucoma. As the first in-depth study of fundus \& OCT multi-modality glaucoma grading, we believe the GAMMA Challenge will be an essential starting point for future research.

==> supply.tex <==
\begin{document}

\section *{Supplementary Material}
In the following sections, we briefly introduce the methods proposed for the auxiliary tasks. The final ranking of the teams considering all three tasks is also reported.

\subsection *{Fovea Localization}
The ranking of fovea localization task is shown in Table \ref{tab:fovea_result}. The results are evaluated by the fovea localization score (see Section \ref{challenge_evaluation}) and Euclidean distance (ED). Teams are ranked by the fovea localization score. The methods of the teams are summarized in Table \ref{tab:fovea_method}. Analogously to the glaucoma grading task, we also implemented a baseline for fovea localization task, which is shown in Figure \ref{fig:loc}. The input of the network is the whole fundus image, and the output is a 2D vector indicating the coordinate of the fovea center. The backbone of the network is ResNet50 and is supervised by the combination of Euclidean distance and MSE loss.

\begin{table}[h]
\centering
\caption{Fovea localization ranking in the GAMMA Challenge.}
\begin{tabular}{c|c|cc}
\hline
\multirow{2}{*}{Rank} & \multirow{2}{*}{Team} & \multirow{2}{*}{Score} & \multirow{2}{*}{ED} \\
                      &                       &                        &                     \\ \hline
1                     & DIAGNOS-ETS           & 9.60294                & 0.00413             \\
2                     & IBME                  & 9.58847                & 0.00429             \\
3                     & SmartDSP              & 9.57458                & 0.00444             \\
4                     & MedIPBIT              & 9.53757                & 0.00485             \\
5                     & Voxelcloud            & 9.53443                & 0.00488             \\
6                     & EyeStar               & 9.51465                & 0.0051              \\
7                     & WZMedTech             & 9.45846                & 0.00573             \\
8                     & MedICAL               & 9.34639                & 0.00699             \\
9                     & FATRI\_AI             & 9.33749                & 0.0071              \\
10                    & HZL                   & 9.22303                & 0.00842             \\ \hline
\end{tabular}
\label{tab:fovea_result}
\end{table}

On fovea localization task, the methods of the teams varies a lot. In the top-10 teams, SmartDSP, MedIPBIT, WZMedTech processed the task as a coordinate regression task, just like we did in the baseline method. VoxelCloud and DIAGNOS-ETS processed the task as a binary segmentation task. They generated a circle centered on the fovea location. The circle is then taken as the segmentation target for the binary segmentation task. The center of the segmented result is finally taken as the fovea location. Eyestar, IBME and MedICAL processed the task as a heatmap prediction task. They generated the ground-truth heatmap by Gaussian kernel. This strategy is similar to the binary segmentation, except it is supervised by a soft target,  which is a normal distribution centered on fovea location. In contrast, FATRI-AI processed the task as a detection task. They generated a 160\texttimes160 square centered on the fovea location and used a YOLO (\cite{redmon2016you}) network to detect the region.

Almost half of the teams utilized a coarse-to-fine multi-stage strategy, including SmartDSP, EyeStar, MedIPBIT, WZMedTech and MedICAL. Most of them cropped Region Of Interest (ROI) based on the coarse stage predictions. The cropped region is then refined by the later stage. EyeStar proposed a more sophisticated architecture based on this strategy and named it Two-Stage Self-Adaptive localization Architecture (TSSAA). They first cropped multi-scale ROI based on the coarse predictions. Then they fused both multi-scale ROI and coarse-level features using sequential ROI Align layer, concatenation, self-attention modules (\cite{vaswani2017attention}) and Fuse layer. An illustration of TSSAA is shown in Figure \ref{fig:loc}.


\subsection *{OD/OC Segmentation}
The ranking of OD/OC segmentation task is shown in Table \ref{tab:segmentation_result}. The results are evaluated by the two Dice values, vertical optic Cup-to-Disc Ratio (vCDR) and the OD/OC segmentation score (see Section \ref{challenge_evaluation}) in the GAMMA Challenge. Teams are ranked by the OD/OC segmentation score. The methods of the teams are summarized in Table \ref{tab:segmentation_result}. A standard UNet is also adopted as the baseline of the task.

\begin{table}[t]
\centering
\caption{OD/OC segmentation ranking in the GAMMA Challenge.}
\resizebox{0.5\textwidth}{!}{%
\begin{tabular}{c|c|cccc}
\hline
\multirow{2}{*}{Rank} & \multirow{2}{*}{Team} & \multirow{2}{*}{Score} & \multirow{2}{*}{Dice-disc(\%)} & \multirow{2}{*}{Dice-cup(\%)} & \multirow{2}{*}{vCDR} \\
                      &                       &                        &                             &                             &                       \\ \hline
1                     & Voxelcloud            & 8.36384                & 96.25                       & 87.84                       & 0.04292               \\
2                     & DIAGNOS-ETS           & 8.3275                 & 95.96                       & 87.74                       & 0.04411               \\
3                     & WZMedTech             & 8.31621                & 96.11                       & 88.04                       & 0.04538               \\
4                     & HZL                   & 8.30093                & 95.83                       & 88.00                       & 0.04562               \\
5                     & SmartDSP              & 8.28488                & 95.79                       & 88.01                       & 0.04642               \\
6                     & MedICAL               & 8.27264                & 95.75                       & 87.57                       & 0.0464                \\
7                     & IBME                  & 8.2309                 & 95.79                       & 87.66                       & 0.04887               \\
8                     & FATRI\_AI             & 8.18773                & 95.40                       & 86.69                       & 0.04917               \\
9                     & MedIPBIT              & 8.15502                & 95.49                       & 87.67                       & 0.05258               \\
10                    & EyeStar               & 8.07253                & 94.77                       & 85.83                       & 0.05326               \\ \hline
\end{tabular}
%
}
\label{tab:segmentation_result}
\end{table}

\begin{table*}[h]
\centering
\caption{Final ranking in the GAMMA challenge.}
\resizebox{0.9\textwidth}{!}{%
\begin{tabular}{c|c|c|c|c}
\hline
\multirow{2}{*}{Rank} & \multirow{2}{*}{Team} & \multirow{2}{*}{Member}                                                                                                     & \multirow{2}{*}{Institute}                                                                                                       & \multirow{2}{*}{Score} \\
                      &                       &                                                                                                                              &                                                                                                                                  &                        \\ \hline
1                     & SmartDSP              & \begin{tabular}[c]{@{}c@{}}Jiongcheng Li, Lexing Huang, Senlin Cai, \\ Yue Huang, Xinghao Ding\end{tabular}                  & Xiamen University                                                                                                                & 8.88892                \\
2                     & Voxelcloud            & \begin{tabular}[c]{@{}c@{}}Qinji Yu, Sifan Song, Kang Dang, Wenxiu \\ Shi, Jingqi Niu\end{tabular}                           & \begin{tabular}[c]{@{}c@{}}Shanghai Jiao Tong University; Xi'an \\ Jiaotong-Liverpool University; VoxelCloud \\ Inc.\end{tabular} & 8.83127                \\
3                     & EyeStar               & \begin{tabular}[c]{@{}c@{}}Xinxing Xu, Shaohua Li, Xiaofeng Lei, Yanyu \\ Xu, Yong Liu\end{tabular}                          & Institute of High Performance Computing, ASTAR                                                                                   & 8.72345                \\
4                     & IBME                  & Wensai Wang, Lingxiao Wang                                                                                                   & \begin{tabular}[c]{@{}c@{}}Chinese Academy of Medical Sciences and \\ Peking Union Medical College\end{tabular}                  & 8.70783                \\
5                     & MedIPBIT              & \begin{tabular}[c]{@{}c@{}}Shuai Lu, Zeheng Li,Hang Tian,Shengzhu \\ Yang,Jiapeng Wu\end{tabular}                            & Beijing Institute of Technology                                                                                                  & 8.70561                \\
6                     & HZL                   & Shihua Huang, Zhichao Lu                                                                                                     & \begin{tabular}[c]{@{}c@{}}Hong Kong Polytechnic University; \\ Southern University of Science and \\ Technology\end{tabular}    & 8.68781                \\
7                     & WZMedTech             & \begin{tabular}[c]{@{}c@{}}Chubin Ou, Xifei Wei, Yong Peng, \\ Zhongrong Ye\end{tabular}                                     & \begin{tabular}[c]{@{}c@{}}Southern Medical University; Tianjin \\ Medical University; Xinjiang University\end{tabular}          & 8.65384                \\
8                     & DIAGNOS-ETS           & \begin{tabular}[c]{@{}c@{}}Adrian Galdran,Bingyuan Liu,José \\ Dolz,Waziha Kabir,Riadh Kobbi,Ismail Ben \\ Ayed\end{tabular} & ETS Montreal; DIAGNOS Inc.                                                                                                       & 8.59884                \\
9                     & MedICAL               & Li Lin, Huaqing He, Zhiyuan Cai                                                                                              & \begin{tabular}[c]{@{}c@{}}Southern University of Science and \\ Technology\end{tabular}                                         & 8.43841                \\
10                    & FATRI\_AI             & \begin{tabular}[c]{@{}c@{}}Qiang Zhou, Hu Qiang, Cheng Zheng, \\ Tieshan Liu, Dongsheng Lu, Xinting Xiao\end{tabular}        & Suixin (Shanghai) Technology Co., LTD.                                                                                           & 8.27601                \\ \hline
\end{tabular}%
}\label{tab:final_rank}
\end{table*}

Like the fovea localization task, all the teams except HZL adopted a coarse-to-fine multi-stage strategy. Generally speaking, OD ROI will be first obtained through the coarse OD segmentation stage. The cropped OD patches will be sent to a subsequent Fine-grained OD/OC segmentation network to obtain the final result. Different from the others, VoxelCloud utilized the blood vessel information to improve the OC/OD segmentation. They first used a pre-trained model to obtain the fundus images' blood vessel segmentation masks. The vessel masks are then concatenated with fundus images as the input. An illustration of their method is shown in Figure \ref{fig:seg}. 

\subsection *{Final Ranking in the GAMMA challenge}
To encourage the teams participate in all three tasks of the GAMMA challenge, the official final ranking is calculated with the scores from all three competition tasks:
\begin{equation}
\begin{split}
Score = & 0.4 \times Score_{g} + 0.3 \times Score_{f} \\
& + 0.3 \times Score_{m}.
\end{split}
\end{equation}
The published final ranking is shown in Table \ref{tab:final_rank}. The detailed leaderboards can be accessed on the GAMMA challenge website at \url{https://aistudio.baidu.com/aistudio/competition/detail/90/0/leaderboard}.


\begin{figure*}[h]
\centering
\includegraphics[width=1\linewidth]{gamma_sup_loc.png}
\caption{An illustration of TSSAA proposed by EyeStar for fovea localization. TSSAA first predicts a coarse heatmap in the coarse stage. Then multi-scale ROI is cropped from the raw image as the input of the subsequent refine stage. In the refine stage, the coarse-level features will also be aligned and fused again for the final prediction.}
\label{fig:loc}
\end{figure*}

\begin{figure*}[h]
\centering
\includegraphics[width=1\linewidth]{gamma_sup_seg.png}
\caption{The coarse stage of OD/OC segmentation model proposed by VoxelCloud. The blood vessel segmentation results predicted from a pre-trained network will be concatenated as the input for the coarse OD segmentation}
\label{fig:seg}
\end{figure*}



\begin{table*}[!htbp]
\centering
\caption{Summary of the fovea localization methods in the GAMMA Challenge}
\resizebox{\textwidth}{!}{%
\begin{tabular}{c|c|c|c|c}
\cline{1-5} 
Team        & Architecture  & Preprocessing   & Ensemble   & Method                                                                                                                                                                                                                                                                                                                                        \\ \cline{1-5}
SmartDSP    & Efficientnet-b4                                                   &  \makecell{(i) Center crop to 2000\texttimes 2000, \\ padding when height \\or width less than 2000\\ (ii) Resize to 224\texttimes 224\\ (iii) Default Data Augmentation}  & 2-fold esmble by averaging          &  \makecell{Two stages coordinate regression:\\  (i) Coarse localization, \\crop to 512\texttimes 512, \\ (ii) Fine-grained localization.}                                                                                                                                                                                      \\  \cline{1-5} 
VoxelCloud  & TransUNet-like architecture                                       &  \makecell{(i) Remove black background\\ (ii) Pad and resize to 512\texttimes 512\\ (iii) Default Data Augmentation + \\Blur + JPEG compression +\\ GaussNoise + Coarse Dropout}                                     & \makecell{Ensemble the predictions \\of 30 models train with \\different hyper-parameters} & \makecell{Binary segmentation the \\fovea centered circle. \\Using the sum of \\binary cross-entropy loss, \\ SoftDice loss, SSIM loss,\\ IOU loss and L1 loss \\to supervise}                                  \\  \cline{1-5} 

EyeStar     & \makecell{Poposed Two-Stage \\Self-Adaptive\\ localization Architecture\\ (TSSAA)} & \makecell{(i) Resize to 998\texttimes998\\(ii) Crop to 896\texttimes896\\(iii) Resize to 224\texttimes224\\(iiii) Default data augmentation}                                                                                                                                                                                                                                 &                                      &  \makecell{Two stages heatmap prediction:  \\(i) Coarse heatmap prediction, \\crop to multi-scale ROI, \\ (ii) Fine-grained localization fusing \\multi-scale ROI and\\ coarse-level features }                                                                                                                                                                                      \\  \cline{1-5} 
HZL         & \makecell{UNet with \\ EfficientNet Backbone}                                    & \makecell{Fundus: Resize to 1024\texttimes1024\\OCT: Resize to 1024\texttimes1024\\ Default  Data Augmentation} &\makecell{Pick 5 best models on 5 \\ different validation folds.\\ Ensemble the results \\ by taking the average.}                                                                                                                                                                                 & \makecell{A multi-task UNet\\ to jointly learn glaucoma grading, \\ OD/OC segmentation \\ and fovea localization. \\Recurrently run the \\model for coarse-to-fine\\ localization}
\\  \cline{1-5} 

MedIPBIT    &  \makecell{ResNet50 for coarse \\localization\\ ResNet101 for Fine-grained\\ localization}  & Resize to 512\texttimes 512  &                                      & \makecell{Three stages coordinate regression:\\ (i) Coarse localization, crop to ROI \\(ii) Sequential two-stage \\Fine-grained localization.} \\  \cline{1-5} 
IBME        &  \makecell{UNet with EfficientNetB5 \\backbone}  &  \makecell{(i) Padding to 2000\texttimes2992 \\(ii) Default Data Augmentation}    &        & \makecell{End-to-end heatmap prediction \\with maximization likelihood \\for the localization} \\  \cline{1-5} 
WZMedTech   &    \makecell{HDRNet (\cite{xie2020end})\\ for the first \\and second stage\\ ResNet50 for the third stage} & \makecell{(i) Center crop to 1920\texttimes1920 \\(ii) Resize to 224\texttimes224 \\(iii) Default Data Augmentation}   &                                      & \makecell{Three stages coordinate regression, \\predicted ROI of last \\stage is cropped as\\ the input of the next stage} \\  \cline{1-5} 
DIAGNOS-ETS &  Double stacked W-Net   &    \makecell{ (i) Resize to 512\texttimes512\\ (ii) Default data augmentation + \\Color Normalization}  & 4-fold temperature ensemble    & \makecell{End-to-end binary segmentation \\the fovea centered circle} \\  \cline{1-5} 
MedICAL     & \makecell{ResNet50 for coordinate \\regression branch\\ EfficientNet-B0 for heatmap \\predication branch}  &  \makecell{(i) Pick G channel of RGB image \\ (ii) Histogram equalization \\(iii) Default data augmentation}  & \makecell{Ensemble the results of \\heatmap branch and\\ coordinate regression branch. \\ If Euclidean distance of \\them larger than 30,\\ take the regression result. \\If else, take the average of \\two results}    & \makecell{Two stages: (i)  Coarse OD/Macular \\segmentation, crop ROI to \\128\texttimes128 and 256\texttimes256 \\ (ii) Feed 128\texttimes128 patches and\\ 256\texttimes256 patches\\to a heatmap predication \\network and coordinate regression\\ network respectively,\\ fuse the results of two branches \\for the final predication} \\ \cline{1-5} 
FATRI-AI    & YOLOv5s (\cite{redmon2016you})       & \makecell{(i) Crop black background \\ (ii) Default data augmentation \\+ Mosaic (\cite{chen2020dynamic})\\ + Cutout} &                                      & \makecell{End-to-end macular \\region detection,\\ macular region is generated by \\a 160\texttimes 160 square \\centered on fovea location}  \\  \cline{1-5} 
\end{tabular}%
}
\label{tab:fovea_method}
\end{table*}


\begin{table*}[!htbp]
\centering
\caption{Summary of the OD/OC segmentation methods in the GAMMA Challenge}
\resizebox{\textwidth}{!}{%
\begin{tabular}{c|c|c|c|c}
\hline
Team        & Architecture                                                                                                                                                          & Preprocessing                                                                                                                                                                    & Ensemble                                                                                                                                                                                                                  & Method                                                                                                                                                                                                                                                                                                \\ \hline
SmartDSP    &  \makecell{DeepLabv3 with ResNet34 \\encoder for coarse \\segmentation DeepLabv3 with \\EfficientNet-b2 encoder for\\ Fine-grained segmentation}  &  \makecell{(i) Crop to 512\texttimes 512 centered \\on the highest brightness point\\ (ii) Default Data Augmentation}                                           & 2-fold ensemble by averaging                                                                                                                                                                                             &  \makecell{Two stages:  (i) Coarse OD \\segmentation, cropping\\  (ii) Fine-grained OD/OC segmentation}                                                                                                                                                                        \\ \hline
VoxelCloud  &  \makecell{TransUNet-like architecture \\for coarse segmentation\\  CENet, TransUNet and Segtran \\for Fine-grained segmentation}                &  \makecell{(i) Resize to 512\texttimes 512\\ (ii) Default data augmentation}                                                                                    &  \makecell{5-fold ensemble by \\averaging for coarse segmentation\\  Ensemble the predictions of \\five folds, three networks and \\two kinds of input by\\ averaging for Fine-grained \\segmentation}    &  \makecell{Two stages: (i) Coarse OD \\segmentation taking blood vessel\\ mask concatenated fundus \\image as input, cropping\\  (ii) Fine-grained OD/OC segmentation \\taking cropped patches \\and polar transformed \\patches as inputs.\\ Model supervised by \\BCE loss + Dice loss}  \\ \hline

EyeStar     & \makecell{Segtran (\cite{li2021medical}) with \\EfficientNet-B4 backbone}                                                                                                                                 &  \makecell{(i) Crop to 576\texttimes576 disc \\region by \\MNet DeepCDR (\cite{fu2018joint}) \\ (ii) Resize to 288\texttimes288\\ (iii) Default data augmentation}  &                                                                                                                                                                                                                          & \makecell{Two stages: (i) Coarse OD \\segmentation using \\ CNN, cropping\\  (ii) Fine-grained OD/OC segmentation \\using Segtran}                                                                                                                                                                                                                                                                                                    \\ \hline
HZL         & \makecell{UNet with \\ EfficientNet Backbone}                                    & \makecell{Fundus: Resize to 1024\texttimes1024\\OCT: Resize to 1024\texttimes1024\\ Default  Data Augmentation} &\makecell{Pick 5 best models on 5 \\ different validation folds.\\ Ensemble the results \\ by taking the average.}                                                                                                                                                                                 & \makecell{A multi-task UNet\\ to jointly learn glaucoma grading, \\ OD/OC segmentation \\ and fovea localization.\\ FAM (\cite{huang2021fapn}) is \\adopted for \\the better segmentation } \\ \hline
MedIPBIT    &  \makecell{CNN-Transformer Mixed UNet\\ CNN backbone implemented \\by ResNet34}                                                              & Resize to 512\texttimes512                                                                                                                                                                &                                                                                                                                                                                                                          &  \makecell{Two stages:  (i) Coarse OD\\ segmentation, cropping\\  (ii) Fine-grained OC segmentation}                                                                                                                                                                           \\ \hline
IBME        &  \makecell{UNet with \\EfficientNetB3 backbone \\for OC center localization\\ UNet with \\EfficientNetB6 backbone \\for Fine-grained segmentation}   & Default data augmentation                                                                                                                                                        &                                                                                                                                                                                                                          &  \makecell{Two stages:  (i) OC center \\localization, crop ROI \\to 512\texttimes 512\\  (ii) Fine-grained OD/OC segmentation}                                                                                                                                                           \\ \hline
WZMedTech   &  \makecell{DeepLabV3 for\\ coarse segmentation\\ TransUNet for\\ Fine-grained segmentation}     &  \makecell{(i) Center crop to 1920\texttimes 1920\\ (ii) Default data augmentation }                                                                          &  \makecell{In the Fine-grained stage, \\ensemble the models supervised\\ by cross-entropy loss  + \\boundary loss + dice loss\\ and that supervided by focal loss + \\dice loss by taking the average}  &  \makecell{Two stages:  (i) Coarse OD \\segmentation, crop ROI \\to 512\texttimes 512\\  (ii) Fine-grained OD/OC segmentation}                                                                                                                                                           \\ \hline
DIAGNOS-ETS & Double stacked W-Net                                                                                                                                                  &  \makecell{(i) Resize to 512\texttimes512\\ (ii) Default data augmentation + \\Color normalization}                                                              &  \makecell{In coarse OD segmentation: \\4-fold ensemble by taking average\\ In Fine-grained OD/OC segmentation: \\4-fold temperature ensemble}                                                      &  \makecell{Two stages:  (i) Coarse OD \\segmentation, crop ROI \\to 512\texttimes 512\\  (ii) Fine-grained OD/OC segmentation}                                                                                                                                                           \\ \hline
MedICAL     & \makecell{UNet with EfficientNet-B4 \\backbone}                                                                                                                                    &  \makecell{(i) Resize to 512\texttimes512\\ (ii) Default data augmentation}    &                                    &  \makecell{Three stages: (i) Coarse OD/Macular\\ segmentation, crop OD ROI \\to 448\texttimes448\\ (ii) Fine-grained OD/OC segmentation, \\crop OC ROI TO 256\texttimes256\\ (iii) Fine-grained OC segmentation}  \\ \hline
FATRI-AI    &  \makecell{YOLOv5s for coarse segmentation\\ HRNet for Fine-grained segmentation}                                                            &  \makecell{(i) Resize to 608\texttimes608\\  (ii) Default data augmentation \\+ Mosaic (\cite{chen2020dynamic})\\ + Cutout}                                                           &                                                                                                                                                                                                                          &  \makecell{Two stages: (i) Coarse OD \\segmentation, crop ROI \\to 512\texttimes 512\\  (ii) Fine-grained OD/OC segmentation. \\Final results will be \\smoothed as ellipses}                                                                                                               \\ \hline
\end{tabular}%
}
\label{tab:segmentation_method}
\end{table*}
\bibliographystyle{model2-names.bst}\biboptions{authoryear}
\bibliography{refs}
\clearpage

\end{document}
